Privately Learning Subspaces

Private data analysis suffers a costly curse of dimensionality. However, the data often has an underlying low-dimensional structure. For example, when optimizing via gradient descent, the gradients often lie in or near a low-dimensional subspace. If that low-dimensional structure can be identified, then we can avoid paying (in terms of privacy or accuracy) for the high ambient dimension. We present differentially private algorithms that take input data sampled from a low-dimensional linear subspace (possibly with a small amount of error) and output that subspace (or an approximation to it). These algorithms can serve as a pre-processing step for other procedures.

==> extra.tex <==
\section{Approximate case}

What if the points are only close to a subspace?

\subsection{TV distance between 1-d gaussians}
%By [\url{https://arxiv.org/pdf/1810.08693.pdf} Thm.~1.1], \[ \mathrm{d}_{\mathrm{TV}} (\mathcal{N}(0,\Sigma_1),\mathcal{N}(0,\Sigma_2) = \Theta\left(\sqrt{\sum_i^d \lambda_i^2}\right),  \]
where $\lambda_1, \cdots, \lambda_d$ are the eignenvalues of $\Sigma_1^{-1} \Sigma_2 - I$.

In our setting $\Sigma_1 = xx^T + \gamma I$ and $\Sigma_2 = yy^T + \gamma I$.

%By [\url{https://en.wikipedia.org/wiki/Sherman-Morrison_formula}], \[\Sigma_1^{-1} = (\gamma I + xx^T)^{-1} = \gamma^{-1} I - \frac{\gamma^{-1} I x x^T \gamma^{-1} I}{1 + x^T \gamma^{-1} I x} = \gamma^{-1} I - \frac{\gamma^{-2}}{1 + \gamma^{-1} \|x\|_2^2} xx^T.\]
Thus 
\begin{align*}
    \Sigma_1^{-1} \Sigma_2 - I &= \left( \gamma^{-1} I - \frac{\gamma^{-2}}{1 + \gamma^{-1} \|x\|_2^2} xx^T \right) \left( \gamma I + yy^T \right) - I\\
    &=\frac{\gamma^{-1}}{1 + \gamma^{-1} \|x\|_2^2} \left( (1 + \gamma^{-1} \|x\|_2^2)yy^T -  xx^T - \gamma^{-1} \langle x, y\rangle xy^T \right)\\
    &=\frac{\gamma^{-1}}{1 + \gamma^{-1} \|x\|_2^2} \left( yy^T -  xx^T + \gamma^{-1} \left( y x^Tx y^T - x x^Ty y^T\right)\right)\\
\end{align*}

\subsection{Case: $k\leq2$}

Algorithm:
\begin{enumerate}
    \item Truncate all points to within a ball of radius
        $O(\sqrt{d\log(n)})$.
    \item Choose reference points $p_1,p_2$ uniformly at
        random on $\cS^{d-1}$.
    \item Randomly partition the dataset into subsets of
        size $k=2$.
    \item For each subset $\{X_{2i},X_{2i+1}\}$:
        \begin{itemize}
            \item Normalise the data points to get
                $Y_{2i},Y_{2i+1}$ respectively.
            \item Project $p_1,p_2$ on to the subspace spanned
                by $Y_{2i},Y_{2i+1}$, and the origin.
            \item Let $Z_i$ be the $kd$-dimensional vector
                containing the projected points.
        \end{itemize}
    \item Run private histograms with randomised offset to collect
        the two clusters.
    \item Truncate all $Z_i$'s to within the nearest histogram
    cluster.
    \item Return the noisy empirical mean of all the $Z_i$'s.
\end{enumerate}

The following definition characterises what good pairs of
points are. A good pair is essentially a pair of points where
both points are far enough from the origin, and their respective
normalised projections with respect to the parameter subspace
are also far from one another.
\begin{definition}[$(\tau,\Pi)$-Aligned Points]
    Let $p_1,p_2 \in \R^d$ and let $\Pi$ be a $k$-dimensional
    subspace of $\R^d$. Suppose $p'_1,p'_2$ are their respective
    projections on to $\Pi$, and $p''_1,p''_2$ are $p'_1,p'_2$
    respectively on being normalised. We say that $p_1,p_2$
    are $(\tau,\Pi)$-aligned if $\|p_1\|,\|p_2\| \geq \tau$,
    $\|p''_1-p''_2\| \geq \tau$ and $\|p''_1+p''_2\| \geq \tau$.
    When the context is clear, we get rid of $(\tau,\Pi)$
    for brevity.
\end{definition}

This definition characterises points if their projections on
to the parameter subspace could be potentially collinear using
sectors of a circle.
\begin{definition}[$(\tau,\Pi)$-Collinear Set]
    Let $S=\{p_1,p_2\}$ be a set of unit vectors, and let $\Pi$
    be a $2$-dimensional subspace of $\R^d$. Suppose $p'_1,p'_2$
    are their respective projections on to $\Pi$, and
    $p''_1,p''_2$ are $p'_1,p'_2$ respectively on being normalised.
    Suppose we divide the unit circle around the origin
    in $\Pi$ into sectors of maximum width $\sqrt{\tau}$.
    We say that $S$ is collinear if $p_1,p_2$ lie in sectors,
    where collinearity of $p_1,p_2$, and the origin is possible.
\end{definition}
Rephrase the last sentence of the definition.

\begin{lemma}
    Let $\Pi$ be a $k$-dimensional subspace of $\R^d$,
    and $p_1,p_2\in\mathcal{S}^{d-1}$ be random unit vectors.
    Then with probability at least $BLAH$, $p_1,p_2$ are
    $(\tau,\Pi)$-aligned.
\end{lemma}
\begin{proof}
    Enough to prove that (1) the points are
    at least $\tau$ far from the origin (easy to generalise
    to $k>2$), and (2) $\{p_1,p_2\}$ is not $(\tau,\Pi)$-collinear.
\end{proof}

\begin{corollary}
    Reference points are aligned with respect to the true
    subspace.
\end{corollary}

\begin{lemma}
    Let $x,y \in \R^d$, such that $\langle x,y \rangle = 0$,
    and let $p_1,p_2 \sim \cN(0,x^Tx + y^Ty + \gamma \id)$.
    Suppose $\Pi$ is the subspace spanned by $x,y$. Then with
    probability at least $BLAH$, $p_1,p_2$ are $(\tau,\Pi)$-aligned.
\end{lemma}
\begin{proof}
    Enough to prove that (1) the points are
    at least $\tau$ far from the origin using the PDF of
    a two-dimensional Gaussian (easy to generalise
    to $k>2$), and (2) $\{p_1,p_2\}$ is not $(\tau,\Pi)$-collinear.
\end{proof}

\begin{corollary}
    At least half the subsets are aligned with respect to
    the true subspace and are at most $O(\gamma\sqrt{d})$
    from their projections on the true subspace.
\end{corollary}
\begin{proof}
    Chernoff bound for the first part. For the second part,
    apply Gaussian tail bound for remaining $d-k$ directions
    for all $n$ points.
\end{proof}

\begin{definition}[$\tau$-Close Subspaces]
    Let $\Pi_1,\Pi_2$ be subspaces of $\R^d$ with the same
    dimensions. Let $p$ be an arbitrary point in the unit
    ball around the origin. We say that $\Pi_1,\Pi_2$ are
    $\tau$-close if for any such $p$,
    $\|\Pi_1 p - \Pi_2 p\| \leq \tau$.
\end{definition}

\begin{lemma}
    Let $\Pi_1$ be a subspace, and $p_1,p_2$ be
    $(\tau,\Pi_1)$-aligned. Suppose $p'_1,p'_2$ are their
    respective projections on to $\Pi_1$, and
    $\|p_i-p'_i\| \leq \tau$ for $i = 1,2$. If $\Pi_2$
    is the subspace spanned by $p_1,p_2$, and the origin,
    then $\Pi_1,\Pi_2$ are $\tau\sqrt{d}$-close.
\end{lemma}
\begin{proof}
    Geometry. EZ PZ.
\end{proof}

\begin{corollary}
    Let $x,y \in \cS^{d-1}$, such that $\langle x,y \rangle = 0$,
    and let $X_1,\dots,X_n \sim \cN(0,x^Tx + y^Ty + \gamma \id)$.
    Suppose $\Pi$ is the subspace spanned by $x,y$, and the origin.
    Let $\{X_1,X_2\},\dots,\{X_{n-1},X_n\}$ be disjoint subsets.
    Then with probability at least $BLAH$, the subspaces spanned
    by at least half of the subsets (and the origin) are
    $\tau\sqrt{d}$-close to $\Pi$.
\end{corollary}

\begin{lemma}
    Let $\wh{Z}$ be the empirical mean of all the $Z_i$'s in the
    algorithm. Then the sensitivity of $\wh{Z}$ is
    square root of twice the size of a single cluster, over $n$.
\end{lemma}

\begin{lemma}
    With probability at least BLAH, there are two histogram clusters, and the ``size'' of each histogram cluster is at most $BLAH$.
\end{lemma}

\section{Approximate case}

Let $X_1, \cdots, X_m \gets \mathcal{N}(0,\sum_i^k u_i u_i^T)$, where $\langle u_i, u_j \rangle = \mathbb{I}[i=j]$ for all $i,j \in [k]$. Let $\xi_1, \cdots, \xi_m \gets \mathcal{N}(0,\gamma I)$. Assume everything is independent. Let $\tilde{X}_i = X_i + \xi_i$ for all $i \in [m]$.

Let $Y \gets \mathcal{N}(0,I)$ be independent from everything else. Let $\hat{Y}$ be the projection of $Y$ onto the space spanned by $u_1, \cdots, u_k$. Note that $\hat Y$ has the same distribution as $X_i$ and that $\hat Y$ is also the projection of $Y$ onto the space spanned by $X_1, \cdots, X_m$. 

Let $\tilde Y$ be the projection of $Y$ onto the space spanned by $\tilde{X}_1, \cdots, \tilde{X}_m$. We wish to show that $\|\hat{Y} - \tilde{Y}\|$ is small on average.



That is, $\hat Y = X(X^TX)^{-1}X^TY$ and $\tilde Y = \tilde{X}(\tilde{X}^T\tilde{X})^{-1}\tilde{X}^TY$. Here $X \in \mathbb{R}^{d \times m}$ is the matrix with $X_1, \cdots, X_m \in \mathbb{R}^d$ as columns.

\begin{comment}
We have $\hat Y = \sum_i^m \alpha_i X_i$ and $\tilde Y = \sum_i^m \tilde\alpha_i \tilde{X}_i$ for appropriate weights. Now 
\begin{align*}
    \|\hat{Y} - \tilde{Y}\| &= \left\|\sum_i^m \alpha_i X_i -\tilde\alpha_i \tilde{X}_i\right\|\\
    &= \left\|\sum_i^m (\alpha_i -\tilde\alpha_i) X_i - \tilde\alpha_i \xi_i\right\|\\
    &\le \sum_i^m |\alpha_i-\tilde\alpha_i| \cdot \|X_i\| + |\tilde\alpha_i|\cdot\|\xi_i\|
\end{align*}

\begin{conj}
Let $y \in \mathbb{R}^d$. Let $S_1, S_2$ be subspaces of dimension $k$. Let $y_i$ be the projection of $y$ onto $S_i$. Let $y_{i,j}$ be the projection of $y_i$ onto $S_j$. Suppose $\|y_1 - y_{1,2}\|\le \gamma$. Then $\|y_1 - y_2\|\le f(\gamma, k, d, \|y\|)$, where $f$ is ``small'' -- specifically, $\lim_{\gamma\to0} f(\gamma,k,d,r)=0$ for all $k$, $d$, and $r$.
\end{conj}
Conjecture is bad: Suppose $y \in S_2$ and $y$ is orthogonal to $S_1$. Then $y_1=y_{1,2}=0$ and $y_2=y$. So $\gamma=0$ and $\|y_1-y_2\|=\|y\|$.
\end{comment}

